Integrating Symbolic Reasoning into Neural Generative Models for Design Generation

Design generation requires tight integration of neural and symbolic reasoning, as good design must meet explicit user needs and honor implicit rules for aesthetics, utility, and convenience. Current automated design tools driven by neural networks produce appealing designs but cannot satisfy user specifications and utility requirements. Symbolic reasoning tools, such as constraint programming, cannot perceive low-level visual information in images or capture subtle aspects such as aesthetics. We introduce the Spatial Reasoning Integrated Generator (SPRING) for design generation. SPRING embeds a neural and symbolic integrated spatial reasoning module inside the deep generative network. The spatial reasoning module samples the set of locations of objects to be generated from a backtrack-free distribution. This distribution modifies the implicit preference distribution, which is learned by a recursive neural network to capture utility and aesthetics. Sampling from the backtrack-free distribution is accomplished by a symbolic reasoning approach, SampleSearch, which zeros out the probability of sampling spatial locations violating explicit user specifications. Embedding symbolic reasoning into neural generation guarantees that the output of SPRING satisfies user requirements. Furthermore, SPRING offers interpretability, allowing users to visualize and diagnose the generation process through the bounding boxes. SPRING is also adept at managing novel user specifications not encountered during its training, thanks to its proficiency in zero-shot constraint transfer. Quantitative evaluations and a human study reveal that SPRING outperforms baseline generative models, excelling in delivering high design quality and better meeting user specifications.

==> tex/7_addi_info.tex <==


\subsection{Declaration of Competing Interest}
A declaration of competing interest form is included with this work.

\subsection{Submission Declaration}
This work has not been published previously and is not under consideration for publication elsewhere. Its submission for publication is approved by all authors and tacitly or explicitly by the responsible authorities where the work was carried out. If accepted, it will not be published elsewhere in the same form, in English or in any other language, including electronically without the written consent of the copyright-holder.



\subsection{What is, in one or two sentences, the original contribution of this work?}

Our approach (SPRING) integrates symbolic and neural reasoning to generate constrained interior design images. This produces designs that are both guaranteed to meet specifications and standards, while also appearing natural and aesthetically pleasing.

%Both authors contributed equally to the conceptualization, experiments, writing, and editing of this work.

\subsection{Why should this contribution be considered important for the field of Artificial Intelligence? Please confirm where you explain this in the paper?}

Our contribution is important to the field of artificial intelligence because it demonstrates a powerful method in which symbolic and neural methods may be integrated to produce results much better than anything using just one. We showcase the strong points and weak points of each, and show that they can be combined to act as \textit{more than the sum of their parts}. 

This is best exemplified by this excerpt from the introduction:

"Neither neural nor symbolic approaches offer a complete solution on their own, as each has its own set of strengths and weaknesses. Consequently, many meaningful real-world tasks remain outside the reach of current artificial intelligences. A better solution would be the integration of neural and symbolic approaches."

This is further discussed in the section How SPRING Advances the AI Field from the introduction.

%Limit 20000 characters.

\subsection{What is the most closely related work by others, and how does this work differ? Please give 1-3 citations to such papers (not papers that of yours or your co-authors, of course), preferably from outlets such as the AI journal, the Journal of Artificial Research, IJCAI, AAAI, ECAI or some similar quality artificial intelligence venue. Your related work section should discuss the relationship in more detail.}

Mitchener, L., Tuckey, D., Crosby, M., \& Russo, A. (2022). Detect, Understand, Act: A Neuro-symbolic Hierarchical Reinforcement Learning Framework. Machine Learning, 111(4), 1523-1549. https://doi.org/10.1007/s10994-022-06142-7

The method described in this work also utilizes a 3-stage neuro-symbolic approach including perception, reasoning, and action (Detect, Understand, Act). Like our work, this approach leverages neural networks for foundational tasks and symbolic methods for higher-level abstract reasoning. However, our work employs distinct symbolic and neural techniques (supervised learning combined with constraint programming as opposed to RL paired with ILP) and integrates them uniquely to tackle varied challenges. Our approaches are quite different but they share a foundational philosophy.

\xyx{please cite this paper in the main text!} \mj{Done! In Fast and Slow section.}
Grady Booch, Francesco Fabiano, Lior Horesh, Kiran Kate, Jon Lenchner, Nick Linck, Andrea Loreggia, Keerthiram Murugesan, Nicholas Mattei, Francesca Rossi, Biplav Srivastava (2021). Thinking Fast and Slow in AI. Proceedings of the AAAI Conference on Artificial Intelligence 2021, 35(17), 15042-15046.


This AAAI paper proposes a research direction to advance AI which draws inspiration from cognitive theories of human decision-making. The premise is that if we gain insights about the
causes of some human capabilities that are still lacking in AI
(for instance, adaptability, generalizability, common sense,
and causal reasoning), we may obtain similar capabilities in
an AI system by embedding these causal components. Our paper is related to this AAAI paper in the sense that we employ symbolic constraint reasoning for System 2 reasoning while leaving System 1 perception and reasoning to neural networks. We discussed the relationship between our work and the fast and slow decision-making in cognitive science in the related work section. The difference between our work and this AAAI paper is that our work implements a physical system capable of integrating systems 1 and 2 reasoning for design generation, while the AAAI paper describes a grand vision of neuro-symbolic integration.


\xyx{I excluded this one.} \mj{Gotcha.}
Zhang, L., Rao, A., \& Agrawala, M. (2023). Adding Conditional Control to Text-to-Image Diffusion Models. In IEEE International Conference on Computer Vision (ICCV).

This work attacks a similar problem space to us: constrained image generation. Their approach is a purely neural one, where conditioning can be added to large text-to-image diffusion models without breaking them or requiring a massive dataset. This approach is undoubtably useful, but it does not offer the same guarantees of following the constraints as our approach can through a neuro-symbolic approach.

Limit 20000 characters.

\subsection{
AIJ will publish only work that is relevant to AI. It must also be accessible to a wide audience, even if the contribution of the paper is a narrow technical one (i.e. other AI researchers, not necessarily in the same sub-field should be able to appreciate the results and understand the paper's contributions and its relevance to AI).
Your paper will be sent back for revisions or rejected if this is not the case. Answer the following two questions:
}

1. Is your work relevant to AI, and where do you explain the relevance to AI in the paper?
Yes. How SPRING Advances the AI Field from the introduction.


2. Can you confirm that at least the abstract, introduction and conclusion can be appreciated by a general AI audience?
Yes. These sections in-part focus on the abstract picture. They are not overladen with jargon pertaining only to the image generation or interior design fields. 

(Do not submit your paper until you are able to answer "yes" to both these questions.)

\subsection{
AIJ encourages authors to submit additional electronic material (data sets, programs, videos....) which would be published in Science Direct if the paper is accepted (though not in the print version). Please describe here any such material you would make available in this way.}

We would seek to publish a copy of the code used to train and evaluate SPRING. The code is written using PyTorch and several other compatible python libraries. A preliminary version of the code is available on GitHub (\url{https://github.com/arcosin/SPRING-Interior-Design}) capable of basic demonstrations. A more curated version of this will be made available in the same repository after publication.

\subsection{Did the availability of the AI journal for free as detailed at http://aij.ijcai.org/free-access-to-the-ai-journal influence your decision to submit to the AI journal?}

No.

\subsection{
Software co-submission
This journal encourages and enables you to share software that supports your research publication where appropriate, and enables you to interlink the software and data with your published article. You have the option to convert your open source software into an additional journal publication in Software Impacts, a multi-disciplinary open access journal that provides a scholarly reference to software that has been used to address a research challenge. It ensures that your software is actively reviewed, curated, formatted, indexed, given a DOI and publicly available to all upon publication. You are encouraged to submit your article to Software Impacts as an additional item If your research article is accepted. Please note an open access fee of 250 USD is payable for publication in Software Impacts. Full details can be found on the Software Impacts guide for authors. Please use this template to write your Software Impacts article.}

\xyx{I select the choice ``Yes, I will submit one article to software impact''?}
\mj{Sounds good. It would help us curate the code.}

\subsection{
Do you have any related research objects (data, methods, protocols, software, hardware) that you would like to publish alongside your original research as an additional paper in Research Elements?
}


Research Elements is a suite of Open Access journals, with associated APCs (article processing charges), which make research objects findable, accessible, and reusable. Manuscripts can be prepared by any member of the team who worked on the original research and submitted at any time.

\xyx{which one should I select? Yes, 
No, 
Not sure, I’d like to learn more?
}
\mj{I think no. The Software Impacts one is enough. We don't have all that much which falls under this besides code anyways.}

\subsection{To complete your submission you must select a statement which best reflects the availability of your research data/code. IMPORTANT: this statement will be published alongside your article. If you have selected "Other", the explanation text will be published verbatim in your article (online and in the PDF).
(If you have not shared data/code and wish to do so, you can still return to Attach Files. Sharing or referencing research data and code helps other researchers to evaluate your findings, and increases trust in your article. Find a list of supported data repositories in Author Resources, including the free-to-use multidisciplinary open Mendeley Data Repository.)
}

See the response in the editorial manager website.

\xyx{Should I select ``Data will be made available on request''?}
\mj{Yes. That is fine.}

\subsection{Funding Sources}

This research was supported by NSF grants IIS-1850243, CCF-1918327. 

No funding source had any role in study design; in the collection, analysis and interpretation of data; in the writing of this report; or in the decision to submit this article for publication.




==> tex/coverletter.tex <==



Reviewer 3 helpfully reminded us to add a citation for Stable Diffusion on page 4. This has been added.

Reviewer 3 noted that content on page 11 includes repetition of what is explained in later pages, and suggests a specific rewrite in which this information is merged into the later sections. 
This recommendation has been taken, and these parts previously under the methodology header have been integrated into their respective subsections with reduced repetition.

Reviewer 3 requested that we rewrite the sections 5.5.1 to 5.5.4 to be more concise.
In 5.5.1, details of the specific questions used in the survey were moved to the appendix, leaving only a concise high level description of remaining metrics.
In 5.5.4, all details on study demographics were moved to the appendix, with a short sentence remaining to point readers in that direction should they be interested.

Reviewer 3 requested that the Key conclusions on page 21 not be presented before the results of experiments. 
We have moved these conclusions to a dedicated subsection (5.5) presented after the experiments.

Reviewer 3 reminded us to clearly identify all abbreviations before using them, pointing out a specific example with the spatial reasoning module (SRM) on page 12. 
This instance has been corrected, and the rest of the paper was closely checked to ensure compliance.
The paper uses the acronyms SPRING, DETR, SRM, VEG, RNN, and GRU which are now all identified before their first appearance.
The COCO Dataset (Microsoft COCO: Common Objects in Context) is not identified in such detail to maintain conciseness, but is cited with its full name.



\begin{tabularx}{\textwidth}{|X|X|}
\hline
Reviewer Criticisms & Author Responses \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
 & \\ \hline
On the 41st line of page 4, please include the citation, such as (Rombach et al., 2022), for the "Stable Diffusion model" &  \\ \hline
The content from lines 12-16 on page 11 is repeated in lines 37-40 on page 12. To reduce repetition, the authors can reorganize the text. & Reviewer 3 noted that content on page 11 includes repetition of what is explained in later pages, and suggests a specific rewrite in which this information is merged into the later sections. This recommendation has been taken, and these parts previously under the methodology header have been integrated into their respective subsections with reduced repetition. \\ \hline
Please rewrite the content of sections 5.5.1 to 5.5.4 more concisely. & Reviewer 3 requested that we rewrite the sections 5.5.1 to 5.5.4 to be more concise. In 5.5.1, details of the specific questions used in the survey were moved to the appendix, leaving only a concise high level description of remaining metrics. In 5.5.4, all details on study demographics were moved to the appendix, with a short sentence remaining to point readers in that direction should they be interested. \\ \hline
Key conclusions (page 21) should not be presented before the results of experiments. & Reviewer 3 requested that the Key conclusions on page 21 not be presented before the results of experiments. We have moved these conclusions to a dedicated subsection (5.5) presented after the experiments. \\ \hline
Ensure to identify the abbreviation before using it. For example, SRM (Spatial Reasoning Module) in line 15 on page 12. & Reviewer 3 reminded us to clearly identify all abbreviations before using them, pointing out a specific example with the spatial reasoning module (SRM) on page 12. This instance has been corrected, and the rest of the paper was closely checked to ensure compliance. The paper uses the acronyms SPRING, DETR, SRM, VEG, RNN, and GRU which are now all identified before their first appearance. The COCO Dataset (Microsoft COCO: Common Objects in Context) is not identified in such detail to maintain conciseness, but is cited with its full name. \\ \hline
\end{tabularx}

==> tex/cutpaste.tex <==
=== old text ===
Design requires both flexible and rigid thinking. In interior design, flexible thinking may be used to judge the loosely-defined aesthetic quality of a room, or to intuitively grasp certain customs that go with the design. This is complimentary to rigid thinking, which involves an understanding of rules and logic -- assuring that the design meets any special requirements and remains practical for use. The difficulty of this problem comes not only from embedding a design into image generation, but also from the automatic extrapolation of unspecified elements of the design -- a function of flexible thinking -- while adhering to the parameters that are given. As an example, the design in Figure \ref{fig:functionality} requires the generation of a microwave right of the oven, but does not specify whether the microwave should be above or below the oven. This problem space has notable significance to the field of AI as a whole. To solve abstract design illustration problems, a specific plan must be extracted from the general design and embodied faithfully in an image. A strong connection between reasoning, knowledge, and visual representation is required. Furthermore, this set of problems encompasses many real-world applications. Among them are interior design visualization, architecture visualization … \mj{I need to add more + cite}. This work primarily focuses on the interior design domain.

This work considers automatic design production. In this problem, an existing design (such as an internal kitchen) is given along with user specifications. The AI is asked to alter the existing design to satisfy user needs. % in which an abstract design given by the user must be visualized in the form of a generated image. 
\xyx{For example, in Figure \ref{fig:functionality}, xxx is given, the model is asked to generate yyy..}
%
State-of-the-art generative models are not capable of solving design production problems. While text-to-image and graph-to-image models now give us exciting opportunities for controllable generation, this control is not exact enough to follow a user-given specification in a guaranteed way. 
%These approaches effectively model flexible thinking, but fail when rigid constraints are introduced. This is liable to cause violations of the design. 
Notice the baseline panel of Figure \ref{fig:functionality}, where a scene is generated, but it does not match the prompt. A microwave and black oven are produced, but the microwave is not above the oven and the blue term is assigned to other elements of the scene nebulously, not the microwave. %Alternatively, constraint reasoning approaches have been developed which are capable of finding a satisfying solution to design requirements, but can not easily optimize the overall quality of the extrapolated design, taking into account customs and aesthetics. 

By abstracting away the decisions associated with the abstract design -- namely the positions of objects in the scene -- these can be solved in a structured way using the built-in constraint reasoning of the forward-checker, and the learned knowledge of the iterative refinement network. While knowledge between the objects and knowledge from the background image have an effect on the layout produced, they do not need to be so sophisticated as to generalize perfectly to all objects for constraints as simple as “the chair is left of the bed”. Instead, the forward checker can handle these aspects of the design -- taking a significant load off of what the RNN needs to learn and generalize to. The result of this natural task splitting is not just that the positions within the layout are guaranteed to match the constraints set forth in the design, but that

method which models designs as a set of spatial constraints represented in propositional logic and accepts a background image already including various objects. 

Models that generate high-quality images such as the stable diffusion model already require large training datasets whose sizes are comparable to all images on the web. 
%
However, in those datasets a small fraction of images contain multiple objects in complex spatial relationships. The annotations of 
these relationships are even scarcer. 
%
All these aspects imply it may not be practical to train an end-to-end 
model that generates designs satisfying complex specifications. 
%
Hence, we use constraint-embedded generative models to which are clearly stated in propositional logic. 
%are often well 
Relate to sg2im


with a hidden state initialized by the scene features and updated with all existing objects. At the start of generating each position variable, the hidden state is summed with a vector generated by the variable encoder -- specifying the object class and positional variable. 

The spatial reasoning network assigns probability scores to each decision. 


\textbf{In Summary}, the SPRING approach:
\begin{itemize}
\item Combines low-level visual element generation with high-level spatial reasoning to solve abstract design illustration problems.
\item Provides stable guarantees that conventional scene generation approaches and text-to-image approaches cannot.
\item Is more interpretable than other methods as a result of its constraint reasoning with iterative refinement approach.
\item Produce well-placed, high-quality images embodying user-provided designs.
\end{itemize}


==> tex/ebnf.tex <==


